Detailed Annotations of Chest X-Rays via CT Projection for Report Understanding

In clinical radiology reports, doctors capture important information about the patient's health status. They convey their observations from raw medical imaging data about the inner structures of a patient. As such, formulating reports requires medical experts to possess wide-ranging knowledge about anatomical regions with their normal, healthy appearance as well as the ability to recognize abnormalities. This explicit grasp on both the patient's anatomy and their appearance is missing in current medical image-processing systems as annotations are especially difficult to gather. This renders the models to be narrow experts e.g. for identifying specific diseases. In this work, we recover this missing link by adding human anatomy into the mix and enable the association of content in medical reports to their occurrence in associated imagery (medical phrase grounding). To exploit anatomical structures in this scenario, we present a sophisticated automatic pipeline to gather and integrate human bodily structures from computed tomography datasets, which we incorporate in our PAXRay: A Projected dataset for the segmentation of Anatomical structures in X-Ray data. Our evaluation shows that methods that take advantage of anatomical information benefit heavily in visually grounding radiologists' findings, as our anatomical segmentations allow for up to absolute 50% better grounding results on the OpenI dataset as compared to commonly used region proposals. The PAXRay dataset is available at https://constantinseibold.github.io/paxray/.

==> figures/dataset/dataset_eval2.tex <==
\renewcommand{\arraystretch}{0.5}
\setlength{\tabcolsep}{1pt}

\begin{figure}[b]
    \begin{minipage}[c]{0.49\linewidth}
      \centering
      \includegraphics[trim={0 0 1cm 0},clip,width=\linewidth]{images/LMAOKILLMELATERALLY.png}
      \caption{We show the assessment of radiologists of label categories for \textit{lateral} images in our dataset on a Likert-scale}
    \label{fig:label_eval2}
    \end{minipage}\hfill
    \begin{minipage}[c]{0.49\linewidth}
        \includegraphics[trim={0 0 1cm 0},clip,width=\linewidth]{images/lmaokillme.png}
        \caption{We show the assessment of radiologists of label categories of \textit{frontal} images in our dataset on a Likert-scale}
        \label{fig:label_eval}
    \end{minipage}
\end{figure}


==> figures/dataset/dataset_statistics.tex <==
\renewcommand{\arraystretch}{0.5}
\setlength{\tabcolsep}{1pt}
\addtolength{\belowcaptionskip}{0pt}
\addtolength{\abovecaptionskip}{2pt}



==> figures/methodology/cooccurence.tex <==
\setlength{\abovecaptionskip}{6pt}
\setlength{\belowcaptionskip}{-30pt}
\begin{wrapfigure}{r}{0.575\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/cooccurrence.pdf}
    \caption{Chord diagramm of the co-occurences of \textit{Anatomies} and \textit{Observations} in medical reports for the OpenI dataset}
    \label{fig:chord}
\end{wrapfigure}
% \begin{wrapfigure}{br}{0.5\textwidth}
%   \begin{center}
%     \includegraphics[width=0.48\textwidth]{example-image-a}
%   \end{center}
%   \caption{Birds}
% \end{wrapfigure}

==> sections/literature.tex <==
    https://arxiv.org/pdf/2006.09920.pdf
    https://scontent-frt3-2.xx.fbcdn.net/v/t39.8562-6/101177000_245125840263462_116067228848855[…]3-2.xx&oh=fb611fddbb3e7c30db7ed1fb71ac8a37&oe=617BA3C7
    https://arxiv.org/pdf/1908.06354v1.pdf
    https://openaccess.thecvf.com/content_cvpr_2017/papers/Xiao_Weakly-Supervised_Visual_Grounding_CVPR_2017_paper.pdf
    https://arxiv.org/pdf/1803.06506.pdf
    https://arxiv.org/pdf/1903.11649.pdf
    https://arxiv.org/pdf/1811.11683.pdf
    https://arxiv.org/pdf/2110.03094.pdf
    
        https://openaccess.thecvf.com/content/ICCV2021/papers/Gonzalez_Panoptic_Narrative_Grounding_ICCV_2021_paper.pdf
    https://openaccess.thecvf.com/content/ICCV2021/papers/Deng_TransVG_End-to-End_Visual_Grounding_With_Transformers_ICCV_2021_paper.pdf
    https://openaccess.thecvf.com/content/ICCV2021/papers/Arbelle_Detector-Free_Weakly_Supervised_Grounding_by_Separation_ICCV_2021_paper.pdf
    https://openaccess.thecvf.com/content/CVPR2021/papers/Huang_Look_Before_You_Leap_Learning_Landmark_Features_for_One-Stage_Visual_CVPR_2021_paper.pdf
    https://openaccess.thecvf.com/content/CVPR2021/papers/Liu_Relation-aware_Instance_Refin[…]for_Weakly_Supervised_Visual_Grounding_CVPR_2021_paper.pdf
    https://openaccess.thecvf.com/content/CVPR2021/papers/Wang_Improving_Weakly_Supervised_[…]_by_Contrastive_Knowledge_Distillation_CVPR_2021_paper.pdf

https://www.jstage.jst.go.jp/article/mii/36/3/36_141/_pdf

https://www.hindawi.com/journals/jhe/2020/2785464/

http://db.jsrt.or.jp/eng.php
https://arxiv.org/pdf/2012.15029.pdf
https://arxiv.org/pdf/2105.09937.pdf
https://openaccess.thecvf.com/content/ICCV2021/papers/Zhou_Visual-Textual_Attentive_Sem[…]sistency_for_Medical_Report_Generation_ICCV_2021_paper.pdf

https://arxiv.org/pdf/2007.15778.pdf

==> tables/dataset/dataset_comparison.tex <==
\renewcommand{\arraystretch}{1.2}
\setlength{\belowcaptionskip}{0pt}
\setlength{\abovecaptionskip}{2pt}

\begin{table}[b]
    \centering
    % 
    \begin{minipage}{0.475\linewidth}
    \Large
    \caption{X-ray dataset comparison  }
    \resizebox{\linewidth}{!}{
    
    \begin{tabular}{cccccc}
    \toprule
   Name & \#Images & View & Annotation & \#Classes \\ 
        \midrule
          JSRT \cite{shiraishi2000development} &{247}&Frontal&Masks& 5\\ 
        
         PAXRay (ours) &{882}& \makecell{Frontal/\\ Lateral} &Masks& \textbf{166}\\ 
     \bottomrule
    \end{tabular}
    }\label{tab:dataset_comparison}
    \end{minipage}
    \hfill
    \begin{minipage}{0.475\linewidth}
    \centering
    \caption{Compressed label structure }
    \includegraphics[width=0.85\linewidth]{images/label_distribution-pdf.png}
    % 
    \label{fig:label_overview}
    \end{minipage}
\end{table}



==> tables/dataset/dataset_distances.tex <==
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{5pt}

\begin{table}[!]
    \centering
    \begin{tabular}{ccccc}
    \toprule
    & Domain & Frontal & Lateral & Overall\\
           \midrule
    \multirow{3}{*}{\rotatebox{90}{Proj.}}&Mean   & $0.1875$       &  $0.4151$ & $0.3013$   \\
     & Matsubara~\etal~\cite{matsubara2019generation} & $0.1672$ & $0.3829$ & $0.2751$ \\
     & Ours   &  $\mathbf{0.1599}$ & $\mathbf{0.3813}$ & $\mathbf{0.2706}$ \\
    \midrule
    \multirow{2}{*}{\rotatebox{90}{Ref.}} & Xray Center & $0.0700$ & $0.1412$ & $0.1056$\\
    


    & VOC07~\cite{pascal-voc-2007} & $0.2593$ & $0.5398$& $0.3995$ \\


    \bottomrule
    \end{tabular}
    \caption{Average relative Nearest-Neighbor Distance between projected/reference real images and images in the OpenI~\cite{openi} dataset based on ResNet-50~\cite{he2016deep} features trained on ImageNet~\cite{imagenet}.}
    \label{tab:dataset_distance}
\end{table}


==> tables/experiments/experiments.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> tables/experiments/hitrate_xray.tex <==
\begin{table}[b!]
    \centering
\begin{tabular}{ c c c c c c c}
\toprule
Method & Data & Features & R@1 & R@5 & R@10 & Accuracy\\
\midrule

- & OpenI & - & - & - & - \\
- & OpenI & - & - & - & - \\
- & OpenI & - & - & - & - \\
\bottomrule
\end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
